Efficient Local Planning with Linear Function Approximation

We study query and computationally efficient planning algorithms with linear function approximation and a simulator. We assume that the agent only has local access to the simulator, meaning that the agent can only query the simulator at states that have been visited before. This setting is more practical than many prior works on reinforcement learning with a generative model. We propose two algorithms, named confident Monte Carlo least square policy iteration (Confident MC-LSPI) and confident Monte Carlo Politex (Confident MC-Politex) for this setting. Under the assumption that the Q-functions of all policies are linear in known features of the state-action pairs, we show that our algorithms have polynomial query and computational costs in the dimension of the features, the effective planning horizon, and the targeted sub-optimality, while these costs are independent of the size of the state space. One technical contribution of our work is the introduction of a novel proof technique that makes use of a virtual policy iteration algorithm. We use this method to leverage existing results on $\ell_\infty$-bounded approximate policy iteration to show that our algorithm can learn the optimal policy for the given initial state even only with local access to the simulator. We believe that this technique can be extended to broader settings beyond this work.

==> chapter/deprecated.tex <==
\section{Proof of Theorem~\ref{thm:main_rand}}\label{apx:main_rand}
To facilitate the proof for the case when the probability transition is stochastic, we begin with several useful definitions. First, we still use the definition of $n$-step trajectory $T_{\pi}^n(s, a)$ as in Definition~\ref{def:trajectory}.  Note that when the transition kernel is stochastic, the trajectory $T_{\pi}^n(s, a)$ is a random sequence, and again, by $s' \in T_{\pi}^n(s, a)$ we mean $s'$ is one of the states in the sequence $T_{\pi}^n(s, a)$. Second, we define a concept that we call \emph{novel starting point}.
\begin{definition}\label{eq:novel_starting_point}
Given a policy $\pi$ and a core set $\cC$ with feature matrix $\Phi_{\cC}$, a novel starting point is a state-action pair $(s, a)$ such that the probability that there exists a state $s'\in T_{\pi}^n(s, a)$ and an action $a'\in\cA$ such that
\begin{align}\label{eq:new_dir}
 \phi(s', a')^\top (\Phi_{\cC}^\top\Phi_{\cC} + \lambda I)^{-1} \phi(s', a') > \tau   
\end{align}
is at least $\frac{\beta}{m}$.
\end{definition}
Intuitively, this definition implies that when we start a rollout process in Algorithm~\ref{alg:rollout}, with a relatively high probability, we will discover an uncertain feature direction $\phi(s', a')$. Here, $\beta \in (0, m)$ is a deterministic quantity that we will choose later in the proof. Moreover, we define the following \emph{detection error} event.
\begin{definition}\label{def:detection_failure}
Suppose that $(s, a)$ is a novel starting point, the detection error event is an event when after running $m$ independent rollouts from $(s, a)$, we never observe a state $s'\in T_{\pi}^n(s, a)$ and an action $a'\in\cA$ such that~\eqref{eq:new_dir} holds.
\end{definition}
Therefore, the probability of detection error is at most
\begin{align}\label{eq:prob_detect_failure}
   (1-\frac{\beta}{m})^m \le e^{-\beta}.
\end{align}

According to Lemma~\ref{lem:coreset_size}, we know that our algorithm must terminate. Let $\cC$ be the core set in the final loop. Define event $\cE_1$ as the event when there exists a policy $\pi_k$ during the policy iteration process in Algorithm~\ref{alg:main} such that the core set of the \emph{final loop} $\cC$ contains some novel starting point for $\pi_k$. By the definition of novel starting point, we know that event $\cE_1$ happens only if detection errors happen to all the novel starting points in $\cC$. 
%\nevena{Why all, isn't it enough to have a detection error for one novel starting point?}\dong{In our algorithm, if a core set element is a novel starting point, and the detection error does not happen, then by the definition detection error, we will be able to find a new direction during rollout, then, rollout subroutine will return uncertain, which contradicts with the fact that this is the final loop. In other words, if we want to ensure this to be the final loop, detection error must happen to all the novel starting points so that we won't be able to find new directions.} 
Therefore, by~\eqref{eq:prob_detect_failure}, we have
\begin{align}\label{eq:prob_event_e1}
    \Prob{\cE_1} \le e^{-\beta}.
\end{align}

We proceed to consider another type of error that we call \emph{estimation error}. This is the event when Algorithm~\ref{alg:rollout} returns the $\mathsf{done}$ status but the estimation is not accurate enough for the Q-function value. More specifically, we have the following definition.

\begin{definition}\label{def:est_error}
Given a policy $\pi$, a core set with feature matrix $\Phi_{\cC}$, and an element from the core set $(s, a):=(z_s, z_a)$, $z\in\cC$, denote $\cG$ as the event that Eq.~\eqref{eq:new_dir} does not hold for any $s'\in T_\pi^n(s, a)$ and any $a'\in\cA$. Let $Q_\pi^{\cG}(s, a)$ be the expected discounted $n$-step cumulative rewards conditioned on $\cG$, i.e.,
\[
Q_\pi^{\cG}(s, a) = \E_{T_\pi^n(s, a)|\cG}\left[ \sum_{t=0}^n \gamma^t r(s_t, a_t) \mid s_0=s, a_0=a \right].
\]
Then, an estimation error is defined as the event when
\[
|z_q - Q_\pi^{\cG}(s, a)| > \theta,
\]
where $z_q$ is the estimation output of Algorithm~\ref{alg:rollout}.
\end{definition}
Here $\theta$ is a deterministic quantity that we choose later in the proof. We know that when Algorithm~\ref{alg:rollout} returns the $\mathsf{done}$ status, it averages $m$ i.i.d. rollout sequences to obtain $z_q$, and since the algorithm did not discover a new feature direction, the sequences are sampled according the distribution of $T_\pi^n(s, a)$ conditioned on $\cG$. Then, according to Hoeffding's inequality, we know that the probability of an estimation error is at most $2\exp(-2\theta^2(1-\gamma)^2m)$. Let $\cE_2$ be the event that estimation error happens at least once during the final loop of the algorithm, then by union bound and Lemma~\ref{lem:coreset_size}, we have
\begin{align}\label{eq:prob_event_e2}
    \Prob{\cE_2} \le 2|\cC|K\exp(-2\theta^2(1-\gamma)^2m)\le \frac{2Kd(1+\tau)}{\lambda \tau^2}\exp(-2\theta^2(1-\gamma)^2m).
\end{align}

In the following discussion, we will condition on the event that none of $\cE_1$ or $\cE_2$ happens. We first provide a lemma that shows the accuracy of the Q-function value for an element $z\in\cC$ that is not a novel starting point.
\begin{lemma}\label{lem:q_est_rand}
Let $\pi$ be a policy that we run rollout in an iteration, and suppose that $(z_s, z_a)$ is not a novel starting point for $\pi$. Then, when estimation error does not happen, we have
\begin{align}\label{eq:est_err_true_q}
|z_q - Q_\pi(z_s, z_a)| \le \frac{\gamma^{n+1}}{1-\gamma} + \frac{\beta}{(1-\gamma)m} + \theta.
\end{align}
\end{lemma}
We prove Lemma~\ref{lem:q_est_rand} in Appendix~\ref{apx:q_est_rand}. Suppose that in the $k$-th iteration, none of the elements in $\cC$ is a novel starting point for $\pi_{k-1}$. We obtain the Q-function estimates $z_q$ and concatenate them into the vector $q_{\cC}$. We then compute the least square estimator $w_k = (\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1}\Phi_{\cC}^\top q_{\cC}$, and let $Q_{k-1}(s, a):=w_k^\top \phi(s, a)$. We still use the same definition of $\cH$ as in~\eqref{eq:defH}, which denotes the set of vectors that are close to the subspace spanned by $\Phi_{\cC}$. Similar to Lemma~\ref{lem:est_error}, the following lemma provides a bound on $|Q_{k-1}(s, a) - Q_{\pi_{k-1}}(s, a)|$, $\forall~(s, a)$ such that $\phi(s, a) \in \cH$.
\begin{lemma}\label{lem:est_error_rand}
Suppose that Assumption~\ref{asm:linear_realizability_prox} holds. Then, for any $(s, a)$ pair such that $\phi(s, a) \in \cH$, we have
\[
|Q_{k-1}(s, a) - Q_{\pi_{k-1}}(s, a)| \le b\sqrt{\lambda \tau} +  \big(\epsilon + \frac{\gamma^{n+1}}{1-\gamma} + \frac{\beta}{(1-\gamma)m} + \theta\big) \sqrt{\frac{d(1+\tau)}{\lambda \tau}}.
\]
\end{lemma}
The proof of this lemma follows the same steps as the proof of Lemma~\ref{lem:est_error} in Appendix~\ref{apx:est_error}. The only difference is that we need to replace the upper bound on $|z_q - Q_{\pi_{k-1}}(z_s, z_a)|$ in~\eqref{eq:err_on_coreset} to the right hand side of~\eqref{eq:est_err_true_q}, and thus the upper bound for the $\ell_\infty$ norm of $\xi$ in~\eqref{eq:bound_xi_prox} is changed to $\epsilon + \frac{\gamma^{n+1}}{1-\gamma} + \frac{\beta}{(1-\gamma)m} + \theta$. The rest of the steps stay the same.

Again, by letting $\epsilon=0$, we can also obtain a direct corollary that when Assumption~\ref{asm:linear_realizability} holds, 
\begin{align}\label{eq:est_error_exact_rand}
|Q_{k-1}(s, a) - Q_{\pi_{k-1}}(s, a)| \le b\sqrt{\lambda \tau} +  \big(\frac{\gamma^{n+1}}{1-\gamma}+ \frac{\beta}{(1-\gamma)m} + \theta \big)\sqrt{\frac{d(1+\tau)}{\lambda \tau}}.
\end{align}
Moreover, since Lemma~\ref{lem:est_error_rand} only provides a bound on the approximation error of the Q-functions on $\cH$, we need to use the idea of virtual policy iteration algorithm in order to use standard results for API.

\subsection{Virtual approximate policy iteration with coupling}\label{sec:virtual_api_coupling}
Similar to the deterministic case, we still use virtual approximate policy iteration algorithm to mitigate the problem that we do not have an $\ell_\infty$ approximation bound for the Q-functions. The major difference from the deterministic case is that the generative model in the virtual algorithm needs to be \emph{synced} and \emph{coupled} with the main algorithm, which we explain below. 

The virtual algorithm is defined as follows. At the beginning of each loop of our main algorithm, the virtual algorithm obtains the same core set $\cC$ with the same ordering as the main algorithm. In the virtual algorithm, we let the initial policy be $\tilde\pi_0=\pi_0$. In the $k$-th iteration ($k\ge 1$), the virtual algorithm runs rollouts with $\tilde\pi_{k-1}$ with a virtual generative model. The rollout process is synced with the main algorithm. This means that when the main algorithm starts the $\mathsf{RolloutWithUncertainty}$ subroutine with a core set element $z$ and policy $\pi_{k-1}$, the virtual algorithm also starts rollout with $z$ with policy $\tilde\pi_{k-1}$. Recall that in the subroutine of the main algorithm queries the generative model at most $mn|\cA|$ times. In comparison, the virtual algorithm does not use the uncertainty estimation and make exactly $mn|\cA|$ queries in each subroutine, and always returns an estimation of the Q-function.

When the main algorithm makes its $N$-th query to the generative model with a state-action pair, say $(s_{\text{main}}, a_{\text{main}})$, the virtual algorithm also makes its $N$-th query to the virtual generative model, with a state-action pair, say $(s_{\text{virtual}}, a_{
\text{virtual}})$. We let the two generative models be \emph{coupled}: when they are queried with the same pair, i.e., $(s_{\text{main}}, a_{\text{main}}) = (s_{\text{virtual}}, a_{
\text{virtual}})$, the next states that they return are also the same. In other words, the generative model for the main algorithm samples $s_{\text{main}}'\sim P(\cdot | s_{\text{main}}, a_{\text{main}})$, and the virtual algorithm samples $s_{\text{virtual}}'\sim P(\cdot| s_{\text{virtual}}, a_{
\text{virtual}})$, and $s_{\text{main}}'$ and $s_{\text{virtual}}'$ satisfy the joint distribution such that $\Prob{s_{\text{main}}' = s_{\text{virtual}}'}=1$. In the cases where $(s_{\text{main}}, a_{\text{main}}) \neq (s_{\text{virtual}}, a_{
\text{virtual}})$ or the main algorithm has already returned due to the discovery of a new feature direction, the virtual algorithm samples from $P$ independently from the main algorithm. Note that this setup guarantees that the virtual algorithm has a valid generative model which can sample from the same probability transition kernel $P$.

Now we describe the virtual policy iteration process. In the $k$-th iteration, the virtual algorithm runs $m$ trajectories of $n$-step rollout from each element $z\in\cC$, obtains the empirical average of the discounted return $z_q$ in the same way as in Algorithm~\ref{alg:rollout}. Then we concatenate them, obtain the vector $\tilde{q}_{\cC}$, compute
\begin{align}\label{eq:linear_est_rand}
    \tilde{w}_k = (\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1}\Phi_{\cC}^\top \tilde{q}_{\cC},
\end{align}
and define the virtual Q-function in the same way as in the deterministic case:
\begin{align}\label{eq:virtual_q_rand}
    \tilde{Q}_{k-1}(s, a) :=
    \begin{cases}
    \tilde{w}_{k}^\top \phi(s, a), & \phi(s, a) \in \cH, \\
    Q_{\tilde\pi_{k-1}}(s, a),  & \phi(s, a)  \notin \cH,
    \end{cases}
\end{align}
by assuming the access to the true Q-function $Q_{\tilde\pi_{k-1}}(s, a)$. The next policy $\tilde{\pi}_k$ is defined as the greedy policy with respect to $\tilde{Q}_{k-1}(s, a)$.

Consider the final loop of the algorithm. We have the following result.
\begin{lemma}\label{lem:virtual_api_rand}
In the final loop of the algorithm, all the rollout trajectories in the virtual algorithm are exactly the same as those in the main algorithm, and therefore $w_k = \tilde{w}_k$ for all $1\le k\le K$.
\end{lemma}
\begin{proof}
The proof of this result follows the same logic as the proof of Lemma~\ref{lem:virtual_api}. We notice that since we only consider the last loop, in any iteration, for any state $s$ in all the rollout trajectories in the main algorithm, and all action $a\in\cA$, $\phi(s, a)\in\cH$. In the first iteration, since $\pi_0=\tilde\pi_0$, and the generative models are coupled, we know that all the rollout trajectories are the same, and as a result, all the Q-function estimates are the same, and thus $w_1 = \tilde{w}_1$. If we have $w_k=\tilde{w}_k$, we know that by the definition in~\eqref{eq:virtual_q_rand}, the policies $\pi_k$ and $\tilde{\pi}_k$ always take the same action given $s$ if for all $a\in\cA$, $\phi(s, a)\in\cH$. Again using the fact that the generative models are coupled, the rollout trajectories by $\pi_k$ and $\tilde\pi_k$ are also the same, and thus $w_{k+1}=\tilde{w}_{k+1}$.
\end{proof}

Since $w_k=\tilde{w}_k$, we have the following simple corollaries. First, for any $(s, a)$, define an event $\cG_\pi$ similar to the event in Definition~\ref{def:est_error}, i.e., $\cG_\pi$ is the event when we start from $(s, a)$, run $n$-step rollout and never observe any feature vector outside of $\cH$. From the discussion above, we know $\Prob{\cG_{\pi_k}} = \Prob{\cG_{\tilde{\pi}_k}}$. Second, for similar reason, $Q_{\pi_k}^{\cG}(s, a) = Q_{\tilde\pi_k}^{\cG}(s, a)$, where $Q_\pi^{\cG}(s, a)$ is defined in Definition~\ref{def:est_error}. Third, since the Q-function estimates $z_q$ are the same, conditioned on the event that none of $\cE_1$ and $\cE_2$ happens, following the same steps as in the proof of Lemma~\ref{lem:q_est_rand}, we know that the inequality~\eqref{eq:est_err_true_q} also holds for $\tilde{\pi}_k$. According to Lemma~\ref{lem:est_error_rand}, we know that for any $(s, a)$ such that $\phi(s, a)\in\cH$,
\begin{align}\label{eq:q_gap_virtual_rand}
|\tilde{Q}_{k-1}(s, a) - Q_{\tilde{\pi}_{k-1}}(s, a)| \le b\sqrt{\lambda \tau} +  \big(\epsilon + \frac{\gamma^{n+1}}{1-\gamma} + \frac{\beta}{(1-\gamma)m} + \theta\big) \sqrt{\frac{d(1+\tau)}{\lambda \tau}} := \eta.
\end{align}
Since when $\phi(s, a)\notin \cH$, $\tilde{Q}_{k-1}(s, a) = Q_{\tilde{\pi}_{k-1}}(s, a)$, we know that $\|\tilde{Q}_{k-1}(s, a) - Q_{\tilde{\pi}_{k-1}}(s, a)\|_\infty \le \eta$. Thus, we conclude that conditioned on the event that none of $\cE_1$ or $\cE_2$ happens, the virtual algorithm is an approximate policy iteration algorithm with $\ell_\infty$ bound $\eta$ for the approximation error on the Q-functions. Similar to the case with deterministic transitions, by standard analysis of API, we can obtain
\begin{align}\label{eq:gap_virtual_rand}
  V^*(\rho) - V_{\tilde{\pi}_{K-1}}(\rho) \le \frac{4\eta}{(1-\gamma)^2} + \frac{2\gamma^{K-2}}{(1-\gamma)^2}.  
\end{align}
Similar to the arguments in the deterministic case in Eq.~\eqref{eq:q_to_v}, we can show that $|V_{\tilde{\pi}_{K-1}}(\rho) - V_{{\pi}_{K-1}}(\rho)| \le 2\eta$.
% \dong{Change the following part}
% Let $z_q$ be the Q-function estimate that we obtain when we run rollout $\pi_{K-1}$ from the core set element $(\rho, \pi_{K-1}(\rho))$ in the main algorithm (equivalently, the estimate when we run rollout with $\tilde\pi_{K-1}$ from $(\rho, \tilde\pi_{K-1}(\rho))$ in the virtual algorithm). Then we have
% \begin{align*}
%     |V_{\tilde{\pi}_{K-1}}(\rho) - V_{{\pi}_{K-1}}(\rho)| &= |Q_{\tilde{\pi}_{K-1}}(\rho, \tilde\pi_{K-1}(\rho))- Q_{\pi_{K-1}}(\rho, \pi_{K-1}(\rho))| \\
%     &\le |Q_{\tilde{\pi}_{K-1}}(\rho, \tilde\pi_{K-1}(\rho)) - z_q| + |z_q - Q_{\pi_{K-1}}(\rho, \pi_{K-1}(\rho))|  \\
%     & \le \frac{2\gamma^{n+1}}{1-\gamma} + \frac{2\beta}{(1-\gamma)m} + 2\theta.
% \end{align*}
Combining this with~\eqref{eq:gap_virtual_rand}, we know that
\begin{align}\label{eq:gap_main_rand}
  V^*(\rho) - V_{{\pi}_{K-1}}(\rho) \le \frac{6\eta}{(1-\gamma)^2} + \frac{2\gamma^{K-2}}{(1-\gamma)^2}.  
\end{align}
By union bound,~\eqref{eq:prob_event_e1} and~\eqref{eq:prob_event_e2}, the error probability of the entire algorithm is at most
\begin{align}\label{eq:error_prob}
    \Prob{\cE_1} + \Prob{\cE_2} \le e^{-\beta} + \frac{2Kd(1+\tau)}{\lambda \tau^2}\exp(-2\theta^2(1-\gamma)^2m).
\end{align}
Finally, we choose appropriate parameters. Suppose that Assumption~\ref{asm:linear_realizability} holds, i.e, $\epsilon=0$ in~\eqref{eq:q_gap_virtual_rand}. It can be verified that by choosing $\tau=1$, $\beta = \log(\frac{2}{\delta})$, $\lambda = \frac{\kappa^2(1-\gamma)^4}{400b^2}$, $n=\frac{5}{1-\gamma}\log(\frac{4db}{\kappa(1-\gamma)})$, $\theta = \frac{\kappa^2(1-\gamma)^4}{900b\sqrt{d}}$, $K=2+\frac{2}{1-\gamma}\log(\frac{4}{\kappa(1-\gamma)})$, $m=5\times 10^5 \frac{db^2}{\kappa^2(1-\gamma)^{10}}\log(\frac{8Kd}{\lambda \delta})$, we can ensure that the error probability is at most $1-\delta$ and $V^*(\rho) - V_{{\pi}_{K-1}}(\rho) \le \kappa$. Suppose that Assumption~\ref{asm:linear_realizability_prox} holds. It can be verified that by choosing $\tau=1$, $\beta = \log(\frac{2}{\delta})$, $\lambda = \frac{3\epsilon\sqrt{d}}{b}$, $n=\frac{1}{1-\gamma}\log(\frac{1}{\epsilon(1-\gamma)})$, $\theta=\epsilon$, $K=2 + \frac{1}{1-\gamma} \log\big(\frac{1}{\epsilon^{1/2}b^{1/2}d^{1/4}}\big)$, $m=\frac{1}{2\epsilon^2(1-\gamma)^2}\log(\frac{8Kd}{\lambda \delta})$, then we can ensure that with probability at least $1-\delta$, 
\[
V^*(\rho) - V_{{\pi}_{K-1}}(\rho) \le \frac{c}{(1-\gamma)^2}\sqrt{b\epsilon\sqrt{d}},
\]
for some universal constant $c>0$.

\subsection{Proof of Lemma~\ref{lem:q_est_rand}}\label{apx:q_est_rand}
We use $(s, a)$ to denote the starting point instead of $(z_s, z_a)$. Recall that the definition of $Q_\pi(s, a)$:
\[
Q_\pi(s, a) = \E_{s_{t+1}\sim P(\cdot | s_t, a_t), a_{t+1} \sim \pi(\cdot | s_{t+1})} \left[ \sum_{t=0}^\infty \gamma^t r(s_t, a_t) \mid s_0=s, a_0=a \right],
\]
and define the $n$-step truncated Q-function:
\[
Q_\pi^n(s, a) = \E_{s_{t+1}\sim P(\cdot | s_t, a_t), a_{t+1} \sim \pi(\cdot | s_{t+1})} \left[ \sum_{t=0}^n \gamma^t r(s_t, a_t) \mid s_0=s, a_0=a \right].
\]
Then we have
\begin{align}\label{eq:diff_q_qn}
   |Q_\pi^n(s, a) - Q_\pi(s, a)| \le \frac{\gamma^{n+1}}{1-\gamma}.
\end{align}
Further, denote $\cG$ as the event that Eq.~\eqref{eq:new_dir} does not hold for any $s'\in T_\pi^n(s, a)$ and any $a'\in\cA$, i.e., we do not observe a new direction by running $n$ steps of rollout. Since $(s, a)$ is not a novel starting point, we know that $\Prob{\overline{\cG}} \le \frac{\beta}{m}$. According to law of total expectation
\begin{align*}
    Q_\pi^n(s, a) =  Q_\pi^{\cG}(s, a)\Prob{\cG} + Q_\pi^{\overline\cG}(s, a)\Prob{\overline{\cG}},
\end{align*}
where $Q_\pi^{\cG}(s, a)$ is defined as in Definition~\ref{def:est_error}, and $Q_\pi^{\overline\cG}(s, a)$ is similarly defined as
\[
Q_\pi^{\overline\cG}(s, a) := \E_{T_\pi^n(s, a)|\overline\cG}\left[ \sum_{t=0}^n \gamma^t r(s_t, a_t) \mid s_0=s, a_0=a \right],
\]
which implies
\begin{equation}\label{eq:diff_qn_qg}
| Q_\pi^n(s, a) - Q_\pi^{\cG}(s, a) | = |Q_\pi^{\overline\cG}(s, a) - Q_\pi^{\cG}(s, a)|\Prob{\overline\cG} \le \frac{\beta}{(1-\gamma)m}.
\end{equation}
Since there is no estimation error,
\begin{align}\label{eq:diff_z_qg}
    |z_q - Q_\pi^{\cG}(s, a) | \le \theta.
\end{align}
We can then complete the proof by combining~\eqref{eq:diff_q_qn},~\eqref{eq:diff_qn_qg} and~\eqref{eq:diff_z_qg}.

\section{Problems with optimal design of core set}
We discuss the potential issues with getting an optimal design of the core set $\cC$. We will omit the RL background and only talk about the problem in the language of linear regression with a simplified description. The notation will be different from previous sections.

Suppose that we have a ground truth parameter $w^*\in\R^d$, $\|w^*\|_2\le b$. For any feature $\phi\in\R^d$, we can query a black box and obtain $q$ which satisfies $|q - \phi^\top w^*| \le \epsilon$. Suppose that we have a core set $\cC$ with feature matrix $\Phi_{\cC}\in\R^{|\cC|\times d}$. We also have a features set $\cH$ (an ellipse) that we eventually care about:
\[
\cH := \{\phi \in \R^d :  \phi^\top (\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1} \phi \le \tau \}. 
\]
According to Lemma~\ref{lem:est_error}, we can show that if we query every row in $\Phi_{\cC}$ to the black box and obtain vector $q$ such that $\|q - \Phi_{\cC}w^*\|_\infty \le \epsilon$, then we can ensure that we can learn linear regression coefficients $\hat{w}$ such that for every $\phi\in\cH$,
\[
|\phi^\top(\hat{w} - w^*)| \le \epsilon\sqrt{|\cC|}.
\]
However, since $|\cC|$ can be as large as $\cO(\frac{d}{\lambda})$, this error bound can have dependency on $\lambda$. The question that we want to address is the following: \emph{Is it possible to improve the process of learning $\hat{w}$ so that we can get}
\[
|\phi^\top(\hat{w} - w^*)| \le \epsilon\sqrt{d} \quad \text{for all}~\phi\in\cH?
\]
One potential way is to try to first obtain a (near) optimal design $\cC^*$ (weights $\rho\in\Delta_{\cC}$, size $|\text{supp}(\rho)|\le \cO(d)$) of $\cC$ and then query the black box using elements in $\cC^*$ (the rows with non-zero weights), then learn $\hat{w}$ by weighted linear regression in the same way as Proposition 4.5 in~\cite{lattimore2020learning}. In fact, by letting $G(\rho) = \sum_{\phi\in\text{rows}(\Phi_{\cC})} \rho(\phi)\phi\phi^\top$, we can guarantee that for every $\phi\in\text{rows}(\Phi_{\cC})$, $\phi^\top G(\rho)^{-1}\phi \le 2d$. Using this fact, Proposition 4.5 in~\cite{lattimore2020learning} shows that
\[
|\phi^\top(\hat{w} - w^*)| \le \epsilon\sqrt{d} \quad \text{for all}~\phi\in\text{rows}(\Phi_{\cC}).
\]
However, we want to get this $\epsilon\sqrt{d}$ result for all $\phi\in\cH$. We compare $\phi\in\text{rows}(\Phi_{\cC})$ and $\phi\in\cH$ as below:
\begin{align}
    \phi\in\text{rows}(\Phi_{\cC}) & \Longrightarrow \phi^\top G(\rho)^{-1}\phi \le 2d \label{eq:in_rows}\\
    \phi\in\cH & \Longleftrightarrow
    \phi^\top (\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1} \phi \le \tau \label{eq:in_H}
\end{align}
Therefore, if we want to show the result for all $\phi\in\cH$, we need to show that the two ellipses in~\eqref{eq:in_rows} and~\eqref{eq:in_H} are \emph{similar in some sense}. In other words, we probably need to show that the eigenspaces corresponding to the \emph{small eigenvalues} of $G(\rho)$ and $\Phi_{\cC}^\top \Phi_{\cC} + \lambda I$ are close. However, it's not clear how to show this since $G(\rho)$ is a particularly designed and reweighted covariance matrix of a small subset of the rows in $\Phi_{\cC}$ (so they may be very different?).


\vspace{-0.2in}
\section{Statistical dependency}
\vspace{-0.2in}
We discuss some issues on statistical dependency. The entire algorithm can be considered as a stochastic process that grows the core set $\cC$. Suppose that in the $N$-th loop, we have a core set $\cC_N$, and we run at most $K$ iterations of policy iteration, in each iteration, we run rollouts from all the elements in $\cC_N$ and estimate the Q-functions. If we identify a feature vector $\phi(s, a)\in\cH$:
\[
\cH := \{\phi \in \R^d :  \phi^\top (\Phi_{\cC_N}^\top \Phi_{\cC_N} + \lambda I)^{-1} \phi \le \tau \},
\]
then we increase the core set to $\cC_{N+1}=\cC_N\cup\{(s, a)\}$; otherwise we stop. Lemma~\ref{lem:coreset_size} shows that this process will stop with probability $1$.

\textbf{Question:} suppose that we condition on the event that the $N$-th loop is the ``stopping loop'', what happens to the accuracy of the Q-function estimates?

First, suppose that we have a policy $\pi$ and a starting point $(s, a)$. In a vanilla rollout algorithm where we do not condition on any event, and run $m$ trajectories of $n$-step rollout, without using uncertainty check, and obtain discounted cumulative rewards $q_1,\ldots, q_m$. In this case, we have a distribution over the $n$-step trajectory $T_\pi^n(s, a)$, say $\cD_T$, then we know that each rollout will produce an unbiased estimate of the truncated Q-function $Q^n_\pi(s, a)$, i.e.,
\[
\E_{\cD_T}[q_i] = Q^n_\pi(s, a).
\]
Because the $m$ trajectories are i.i.d. and cumulative reward is always bounded in $[0, 1/(1-\gamma)]$, we can apply Hoeffding to obtain
\[
\Prob{|\frac{1}{m}\sum_{i=1}^m q_i - Q^n_\pi(s, a)| \ge \theta} \le \delta.
\]
Now we \emph{condition} on the event that this rollout process happens in the \emph{stopping loop}. It means that for the $m$ trajectories that we collect, for every state $s$ in the trajectory, and all $a\in\cA$, $\phi(s, a)\in\cH$. We call this a ``good'' event $\cG$. This means that the conditional distribution of the trajectories has changed to certain conditional distribution $\cD_T^\cG$, which is the distribution of the rollout trajectories that do not ``go outside of $\cH$''. The question now is that \emph{can we still argue that the $m$ trajectories are sampled i.i.d. according to $\cD_T^{\cG}$ and apply Hoeffding to get}
\[
\Prob{|\frac{1}{m}\sum_{i=1}^m q_i - Q^{n, \cG}_\pi(s, a)| \ge \theta} \le \delta,
\]
where $Q^{n, \cG}_\pi(s, a)$ is the expected discounted $n$-step reward conditioned on the event that the trajectories do not ``go outside of $\cH$''?

It seems that this kind of ``conditional i.i.d.'' argument still works since the event that we are at a stopping loop is basically equivalent to the event that each trajectory does not ``go outside of $\cH$'', which does not affect that these trajectories are independent and identically distributed (but they are just biased so we get an unbiased estimator of a conditional expectation).

\section{Separating examples?}

\begin{algorithm}[ht]
\caption{$\mathsf{RolloutWithUncertainty}$}
\begin{algorithmic}[1]\label{alg:rollout_v2}
\STATE \textbf{Input:} number of detection rollouts $m_1$, number of estimation rollouts $m_2$, length of rollout $n$, policy parameter $w$, discount $\gamma$, initial state $s_0$, initial action $a_0$, feature matrix $\Phi_{\cC}$, regularization coefficient $\lambda$, threshold $\tau$.
\IF{there exists $a'\in\cA$ such that $\phi(s_{0}, a')^\top (\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1} \phi(s_{0}, a') > \tau$}
\STATE $\status \leftarrow \uncertain$, $\result\leftarrow (s_{0}, a', \phi(s_{0}, a'), \none)$
\STATE \textbf{return~} $\status, \result$
\ENDIF
\FOR{$i=1,\ldots, m_1$}
\STATE $s_{i,0} \leftarrow s_0$, $a_{i, 0} \leftarrow a_0$, query the generative model, obtain reward $r_{i, 0} \leftarrow r(s_{i, 0}, a_{i, 0})$, next state $s_{i, 1}$.
\FOR{$t=1,\ldots, n$}
\STATE Query the generative model with $(s_{i, t}, a)$, $\forall a\in\cA$.
\STATE Obtain rewards $r(s_{i, t}, a)$, feature vectors $\phi(s_{i, t}, a)$, next states $s'_{i, t}(a)$, $\forall a\in\cA$.
\IF{there exists $a'\in\cA$ such that $\phi(s_{i,t}, a')^\top (\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1} \phi(s_{i,t}, a') > \tau$}
\STATE $\status \leftarrow \uncertain$, $\result\leftarrow (s_{i, t}, a', \phi(s_{i, t}, a'), \none)$
\STATE \textbf{return~} $\status, \result$
\ENDIF
\STATE $a_{i, t} \leftarrow \arg\max_{a\in\cA}w^\top \phi(s_{i, t}, a)$, $s_{i, t+1} \leftarrow s'_{i,t}(a_{i, t})$.
\ENDFOR
\ENDFOR
\FOR{$i=1,\ldots, m_2$}
\STATE $s_{i,0} \leftarrow s_0$, $a_{i, 0} \leftarrow a_0$, query the generative model, obtain reward $r_{i, 0} \leftarrow r(s_{i, 0}, a_{i, 0})$, next state $s_{i, 1}$.
\FOR{$t=1,\ldots, n$}
\STATE Query the generative model with $(s_{i, t}, a)$, $\forall a\in\cA$.
\STATE Obtain rewards $r(s_{i, t}, a)$, feature vectors $\phi(s_{i, t}, a)$, next states $s'_{i, t}(a)$, $\forall a\in\cA$.
\STATE $a_{i, t} \leftarrow \arg\max_{a\in\cA}w^\top \phi(s_{i, t}, a)$, $r_{i,t}\leftarrow r(s_{i,t}, a_{i,t})$, $s_{i, t+1} \leftarrow s'_{i,t}(a_{i, t})$.
\ENDFOR
\ENDFOR
\STATE $\status \leftarrow \done$, $\result \leftarrow \frac{1}{m_2}\sum_{i=1}^{m_2} \sum_{t=0}^n \gamma^t r_{i, t}$
\STATE \textbf{return~} $\status, \result$
\end{algorithmic}
\end{algorithm}


\subsection{Subroutine: \initname}
As mentioned, at the beginning of the algorithm, we first draw $n_0$ i.i.d. samples $s_\init^{1}, \ldots, s_\init^{n_0}$ according to the initial state distribution $\rho$. Then, we initialize the core set $\cC$ using these examples with the subroutine \initname. In this subroutine, we first choose an arbitrary action $a\in\cA$ and initialize $
\cC = \{(s_\init^{1}, a, \phi(s_\init^{1}, a), \none)$. Then we enumerate all the state-action pairs $(s_\init^{i}, a)$, $i\in[n_0], a\in\cA$. If $\phi(s_\init^{i}, a)$ is not in the confident set $\cH$ associated with the current feature matrix $\Phi_{\cC}$, then we add this state-action pair to the core set. Note that the confident set grows as we enlarge the core set.\footnote{According to the Sherman–Morrison formula~\citep{sherman1950adjustment}, when we add more rows to the feature matrix $\Phi_{\cC}$, $\phi^\top (\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1} \phi$ does not increase for any $\phi\in\R^d$.} The subroutine is formally presented in Algorithm~\ref{alg:init}. We note that at the end of this initialization subroutine, for any initial state $s_\init^{i}$ and any action $a\in\cA$, the feature $\phi(s_\init^{i}, a)$ is in the confident set $\cH$.

\begin{algorithm}[ht]
\caption{\initname}
\begin{algorithmic}[1]\label{alg:init}
\STATE \textbf{Input:} initial states $s_\init^{i}$, $i\in[n_0]$, regularization coefficient $\lambda$, threshold $\tau$.
\STATE \text{choose an arbitrary} $a\in\cA$, $\cC\leftarrow\{(s_\init^{1}, a, \phi(s_\init^{1}, a), \none)\}$
\FOR{$i=1,\ldots, n_0$}
\FOR{$a\in\cA$}
\IF{$\phi(s_\init^{i}, a)^\top (\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1} \phi(s_\init^{i}, a) > \tau$}
\STATE $\cC\leftarrow \cC \cup \{(s_\init^{i}, a, \phi(s_\init^{i}, a), \none)\}$
\ENDIF
\ENDFOR
\ENDFOR
\STATE \textbf{return} $\cC$.
\end{algorithmic}
\end{algorithm} 


\subsection{Proof of Lemma~\ref{lem:est_error}}\label{apx:est_error}
Since the transition kernel and the policy are both deterministic, by the definition of Q-function and our rollout procedure in Algorithm~\ref{alg:rollout}, we know that for any $z\in\cC$,
\begin{align*}
    z_q &= \sum_{t=0}^n \gamma^t r(s_t, a_t), \quad
    Q_{\pi_{k-1}}(z_s, z_a) = \sum_{t=0}^\infty \gamma^t r(s_t, a_t),
\end{align*}
where $s_0 = z_s$, $a_0=z_a$, $s_{t} \sim P(\cdot | s_{t-1}, a_{t-1})$, $a_t \sim \pi_{k-1}(\cdot | s_{t})$. This implies that for any $z\in\cC$,
\begin{align}\label{eq:err_on_coreset}
    |z_q - Q_{\pi_{k-1}}(z_s, z_a)| \le \frac{\gamma^{n+1}}{1-\gamma},
\end{align}
since the reward $r(\cdot, \cdot)\in[0, 1]$.

Suppose that Assumption~\ref{asm:linear_realizability_prox} holds. We know that there exists $w_{\pi_{k-1}}\in\R^d$ with $\|w_{\pi_{k-1}}\|_2\le b$ such that for any $s, a$, 
\[
|Q_{\pi_{k-1}}(s, a) - w_{\pi_{k-1}}^\top \phi(s, a)|\le \epsilon.
\]
Let $\xi:=q_{\cC} - \Phi_{\cC}w_{\pi_{k-1}}$. Then according to~\eqref{eq:err_on_coreset},
\begin{align}\label{eq:bound_xi_prox}
    \|\xi\|_\infty \le \epsilon + \frac{\gamma^{n+1}}{1-\gamma}.
\end{align}

Suppose that for a state-action pair $s, a$, the feature vector $\phi:=\phi(s, a)\in\cH$, with $\cH$ defined in~\eqref{eq:defH}. Then we have
\begin{align}
    |Q_{k-1}(s, a) - Q_{\pi_{k-1}}(s, a)| & = |\phi^\top w_k  - \phi^\top w_{\pi_{k-1}}|   \nonumber \\
    &= |\phi^\top(\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1}\Phi_{\cC}^\top (\Phi_{\cC}w_{\pi_{k-1}} + \xi) - \phi^\top w_{\pi_{k-1}}|  \nonumber \\
    &\le \underbrace{| \phi^\top \big(I- (\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1}\Phi_{\cC}^\top\Phi_{\cC}\big)w_{\pi_{k-1}} |}_{E_1} + \underbrace{|\phi^\top(\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1}\Phi_{\cC}^\top \xi|}_{E_2}. \label{eq:split}
\end{align}
We then bound $E_1$ and $E_2$ in~\eqref{eq:split}. Similar to Appendix~\ref{apx:coreset_size}, let $\Phi_{\cC}^\top \Phi_{\cC} + \lambda I := V\Lambda V^\top$ be the eigendecomposition of $\Phi_{\cC}^\top \Phi_{\cC} + \lambda I$ with $\Lambda=\diag(\lambda_1,\ldots, \lambda_d)$ and $V$ being an orthonormal matrix. Notice that for all $i$, $\lambda_i \ge \lambda$. Let $\alpha = V^\top \phi$. Then for $E_1$, we have
\begin{align}
    E_1 &= |\phi^\top V \big(I - \Lambda^{-1}(\Lambda - \lambda I) \big) V^\top w_{\pi_{k-1}}| =\lambda |\phi^\top V \Lambda^{-1} V^\top w_{\pi_{k-1}}|  \nonumber \\
    & \le \lambda b \|\alpha^\top \Lambda^{-1}\|_2 = \lambda b\sqrt{\sum_{i=1}^d \frac{\alpha_i^2}{\lambda_i^2}} \nonumber \\
    & \le b\sqrt{\lambda}\sqrt{\sum_{i=1}^d \frac{\alpha_i^2}{\lambda_i}}, \label{eq:bound_e1_1}
\end{align}
where for the first inequality we use Cauchy-Schwarz inequality and the assumption that $\| w_{\pi_{k-1}} \|_2\le b$, and for the second inequality we use the fact that $\lambda_i \ge \lambda$. On the other hand, since we know that $\phi\in\cH$, we know that $\alpha^\top \Lambda^{-1} \alpha \le \tau$, i.e., $\sum_{i=1}^d \alpha_i^2 \lambda_i^{-1} \le \tau$. Combining this fact with~\eqref{eq:bound_e1_1}, we obtain
\begin{align}\label{eq:bound_e1_2}
    E_1 \le b\sqrt{\lambda\tau}.
\end{align}

We now bound $E_2$. According to H\"{o}lder's inequality, we have
\begin{align}
    E_2 &\le \| \phi^\top(\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1}\Phi_{\cC}^\top \|_1 \|\xi\|_\infty  \nonumber \\
    & \le \| \phi^\top(\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1}\Phi_{\cC}^\top \|_2  \|\xi\|_\infty \sqrt{|\cC|}  \nonumber \\
    &=\big( \phi^\top(\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1}\Phi_{\cC}^\top \Phi_{\cC} (\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1} \phi \big)^{1/2} \|\xi\|_\infty \sqrt{|\cC|} \nonumber \\
    &= \big( \alpha^\top \Lambda^{-1}(\Lambda - \lambda I)\Lambda^{-1}\alpha \big)^{1/2} \|\xi \|_\infty \sqrt{|\cC|} \nonumber \\
    &=\sqrt{\sum_{i=1}^d \alpha_i^2 \frac{\lambda_i-\lambda}{\lambda_i^2}} \|\xi \|_\infty \sqrt{|\cC|} \nonumber \\
    &\le  (\epsilon + \frac{\gamma^{n+1}}{1-\gamma}+\theta) \sqrt{\frac{d(1+\tau)}{\lambda \tau}}, \label{eq:bound_e2}
\end{align}
where in the last inequality we use the facts that $\sum_{i=1}^d \alpha_i^2\lambda_i^{-1} \le \tau$, Eq.~\eqref{eq:bound_xi_prox}, and Lemma~\ref{lem:coreset_size}. We can then complete the proof by combining~\eqref{eq:bound_e1_2} and~\eqref{eq:bound_e2}.


\section{Proof of Theorem~\ref{thm:main_det}}\label{apx:main_det}

\begin{theorem}[Deterministic transition]\label{thm:main_det}
Assume that the transition kernel $P$ is deterministic 
and let $m=1$. If Assumption~\ref{asm:linear_realizability} holds, then for an arbitrarily small $\kappa>0$, by choosing $\tau = 1$, $\lambda = \frac{\kappa^2(1-\gamma)^4}{324 b^2}$, $K = 2+\frac{2}{1-\gamma}\log(\frac{3}{\kappa(1-\gamma)})$, and $n=\frac{5}{1-\gamma}\log(\frac{4db}{\kappa(1-\gamma)})$, the policy $\pi$ that Algorithm~\ref{alg:main} outputs satisfies
\[
V^*(\rho) - V_{\pi}(\rho) \le \kappa.
\]
Alternatively, if Assumption~\ref{asm:linear_realizability_prox} holds, then by choosing $\tau=1$, $\lambda = \frac{\epsilon}{b}\sqrt{2d}$, $K=2 + \frac{1}{1-\gamma} \log\big(\frac{1}{\epsilon^{1/2}b^{1/2}d^{1/4}}\big)$, and $n=\frac{1}{1-\gamma}\log(\frac{1}{\epsilon(1-\gamma)})$, the policy $\pi$ that Algorithm~\ref{alg:main} outputs satisfies
\[
V^*(\rho) - V_{\pi}(\rho) \le \frac{24\sqrt{b\epsilon\sqrt{d}}}{(1-\gamma)^2}.
\]
\end{theorem}

Since it has already been shown in Lemma~\ref{lem:coreset_size} that the algorithm terminates within $\frac{d(1+\tau)}{\lambda \tau^2}$ loops, here we focus on the final output loop in Algorithm~\ref{alg:main}. In this loop, we begin with a core set $\cC$, and run $K$ steps of policy iteration. During the policy iteration process, the $\mathsf{RolloutWithUncertainty}$ subroutine always returns the $\mathsf{done}$ status, in other words, the $\mathsf{RolloutWithUncertainty}$ subroutine is never uncertain about the result. After $K$ iterations, the algorithm outputs $w_K$ as the parameter of the final policy.

Recall that in the $k$-th iteration, the algorithm begins with a policy $\pi_{k-1}$ parameterized by $w_{k-1}$.
Let $Q_{\pi_{k-1}}$ be the true Q-function for $\pi_{k-1}$. According to Algorithm~\ref{alg:main}, we estimate $Q_{\pi_{k-1}}$ using a function that is linear in the features $\phi(s,a)$, i.e., $Q_{k-1}(s, a) := w_k^\top \phi(s, a)$, and then the new policy $\pi_k$ is greedy with respect to $Q_{k-1}$. We summarize this process below:
\begin{align}\label{eq:api}
    \pi_0 \xrightarrow[]{\text{approx Q}} Q_0 \xrightarrow[]{\text{greedy}} \pi_1 \xrightarrow[]{\text{approx Q}} Q_1 \xrightarrow[]{\text{greedy}} \pi_2 \xrightarrow[]{\text{approx Q}} \cdots \xrightarrow[]{\text{greedy}} \pi_K.
\end{align}
We observe that by the algorithm design, $Q_{k-1}$ is only guaranteed to be close to the true Q-function $Q_{\pi_{k-1}}$ when the feature vector is close to the subspace spanned by $\Phi_{\cC}$. More precisely, define
\begin{align}\label{eq:defH}
  \cH := \{\phi \in \R^d :  \phi^\top (\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1} \phi \le \tau \}.  
\end{align}
The following lemma provides a bound on $|Q_{k-1}(s, a) - Q_{\pi_{k-1}}(s, a)|$, $\forall~(s, a)$ such that $\phi(s, a) \in \cH$.
\begin{lemma}\label{lem:est_error}
Suppose that Assumption~\ref{asm:linear_realizability_prox} holds. Then, for any $(s, a)$ pair such that $\phi(s, a) \in \cH$, we have
\[
|Q_{k-1}(s, a) - Q_{\pi_{k-1}}(s, a)| \le b\sqrt{\lambda \tau} +  \big(\epsilon + \frac{\gamma^{n+1}}{1-\gamma}\big) \sqrt{\frac{d(1+\tau)}{\lambda \tau}}.
\]
\end{lemma}
%{\botao (Botao: I feel this lemma perhaps the main resource that worsens the dependency on $H$ in the sample complexity. If we construct one more optimal design within $\cH$, can we improve $\sqrt{\frac{d(1+\tau)}{\lambda \tau}}$ to $\sqrt{d}$? $\sqrt{\frac{d(1+\tau)}{\lambda \tau}}$ is an upper bound on the size of $\cC$ that enjoys a worse-case fashion. Comparing to the proof of Theorem 6.1 in \cite{lattimore2020learning}, their estimation error is roughly $\varepsilon\sqrt{d}$.)}
We prove Lemma~\ref{lem:est_error} in Appendix~\ref{apx:est_error}. Note that by letting $\epsilon=0$, we can also obtain a direct corollary that when Assumption~\ref{asm:linear_realizability} holds, 
\begin{align}\label{eq:est_error_exact}
|Q_{k-1}(s, a) - Q_{\pi_{k-1}}(s, a)| \le b\sqrt{\lambda \tau} +  \frac{\gamma^{n+1}}{1-\gamma}\sqrt{\frac{d(1+\tau)}{\lambda \tau}}.
\end{align}
We notice that since these bounds are only for the feature vectors in $\cH$, it is not sufficient to guarantee the convergence of the approximate policy iteration (API) process in~\eqref{eq:api}.
This is because in standard analysis for API~\citep{munos2003error,farahmand2010error}, requires that $Q_{k-1}$ and $Q_{\pi_{k-1}}$ should be close in some $\ell_p$ norm.
To mitigate this problem, we define a process named \emph{virtual approximate policy iteration} in the next section.

\subsection{Virtual approximate policy iteration}

We define virtual approximate policy iteration using induction. Note that for this process we use the same core set $\cC$ as in our main algorithm.

We begin with $\tilde{\pi}_0:=\pi_0$. Suppose that in the $k$-th iteration, we have a deterministic policy $\tilde{\pi}_{k-1}$. Then for every $z\in\cC$, we start with the state-action pair $(z_s, z_a)$, run $n$-step roll-out using the simulator, get rewards $r_0,\ldots, r_n$, and compute the cumulative discounted reward $z_q :=\sum_{t=0}^n \gamma^t r_t$ as an estimation of $Q_{\tilde\pi_{k-1}}(z_s, z_a)$. Once we have $z_q$ for all $z\in\cC$, we concatenate them and obtain the vector $\tilde{q}_{\cC}$. Then we compute
\begin{align}\label{eq:linear_est}
    \tilde{w}_k = (\Phi_{\cC}^\top \Phi_{\cC} + \lambda I)^{-1}\Phi_{\cC}^\top \tilde{q}_{\cC}.
\end{align}
We define the following \emph{virtual} Q-function
\begin{align}\label{eq:virtual_q}
    \tilde{Q}_{k-1}(s, a) :=
    \begin{cases}
    \tilde{w}_{k}^\top \phi(s, a), & \phi(s, a) \in \cH, \\
    Q_{\tilde\pi_{k-1}}(s, a),  & \phi(s, a)  \notin \cH,
    \end{cases}
\end{align}
where $\cH$ is defined as in~\eqref{eq:defH}. This means that we assume that we have access to the true Q-function of $\tilde\pi_{k-1}$ and when $\phi(s, a)$ is not in $\cH$, the virtual Q-function takes value $Q_{\tilde\pi_{k-1}}(s, a)$. The next policy $\tilde\pi_{k}$ is defined as the greedy policy with respect to $\tilde{Q}_{k-1}(s, a)$. Note that in the virtual algorithm, all the policies are still deterministic; however, we do not require them to take the form~\eqref{eq:greedy_policy}. We summarize the virtual API process as follows:
\begin{align}\label{eq:virtual_api}
    \tilde\pi_0 \xrightarrow[\text{virtualize}]{\text{approx Q}} \tilde{Q}_0 \xrightarrow[]{\text{greedy}} \tilde\pi_1 \xrightarrow[\text{virtualize}]{\text{approx Q}} \tilde{Q}_1 \xrightarrow[]{\text{greedy}} \tilde\pi_2 \xrightarrow[\text{virtualize}]{\text{approx Q}} \cdots \xrightarrow[]{\text{greedy}} \tilde\pi_K.
\end{align}

We now discuss the relationship between our actual algorithm and the virtual algorithm. To facilitate the discussion, we make the following definition.

\begin{definition}\label{def:trajectory}
For a probability transition kernel $P$ and a policy $\pi$, the $n$-step trajectory $T_{\pi}^n(s, a)$ is defined as the sequence $(s_0, a_0, r_0, s_1, a_1, r_1, \ldots, s_n, a_n, r_n)$ with $s_0=s$, $a_0=a$, $r_t=r(s_t, a_t)$, $s_t \sim P(\cdot | s_{t-1}, a_{t-1})$, and $a_t \sim \pi(\cdot | s_t)$ for $1 \le t \le n$.
%The $n$-step feature space starting from $(s, a)$ is defined as $\Phi_{\pi}^n(s, a) = \{\phi(s', a'): s' \in T_{\pi}^n(s, a), a'\in\cA\}$.
\end{definition}

%Notice that in the definition of $\Phi_{\pi}^n(s, a)$, as long as $s'\in T_{\pi}^n(s, a)$, we collect all the feature vectors $\phi(s', a')$, $\forall a'\in \cA$ into $\Phi_{\pi}^n(s, a)$.
Since in this section we only consider deterministic transition and policy, $T_\pi^n(s, a)$ is always a deterministic sequence. With this definition, we can proceed to prove the following property of the virtual approximate policy iteration algorithm.

\begin{lemma}\label{lem:virtual_api}
For all $k$ such that $0\le k \le K-1$, $T_{\pi_{k}}^n(z_s, z_a) = T_{\tilde\pi_{k}}^n(z_s, z_a)$, $\forall z\in\cC$.
\end{lemma}
\begin{proof}
In this proof, by $s' \in T_{\pi}^n(s, a)$ we mean $s'$ is one of the states in the state-action sequence $T_{\pi}^n(s, a)$.
We prove this result by induction. This claim trivially holds for $k=0$ since $\pi_{0} = \tilde\pi_{0}$. Assume this claim holds for $k-1$, i.e., $\forall z\in\cC$, $T_{\pi_{k-1}}^n(z_s, z_a) = T_{\tilde\pi_{k-1}}^n(z_s, z_a)$. Since the estimation of the Q-function values $z_q$ uses the cumulative discounted reward along the trajectories $T_{\pi_{k-1}}^n(z_s, z_a)$ and $T_{\tilde\pi_{k-1}}^n(z_s, z_a)$ for $\pi_{k-1}$ and $\tilde\pi_{k-1}$, respectively, we know that $q_\cC = \tilde{q}_\cC$. Further, since the Q-function approximation uses the same linear estimation as in~\eqref{eq:linear_est}, we know that $w_k = \tilde{w}_k:=w$. Recall the definitions of $\pi_k$ and $\tilde\pi_k$ are
\begin{align*}
    \pi_k(a | s) & = \ind \left(a = \arg\max_{a'\in\cA} w^\top \phi(s, a')\right), \\
    \tilde\pi_k(a | s) & = \ind \left(a = \arg\max_{a'\in\cA} \tilde{Q}_{k-1}(s, a')\right).
\end{align*}
To show that $T_{\pi_{k}}^n(z_s, z_a) = T_{\tilde\pi_{k}}^n(z_s, z_a)$, it suffices to show that $\forall s\in T_{\pi_{k}}^n(z_s, z_a)$, $\pi_{k}(a|s) = \tilde\pi_{k}(a|s)$. According to the definition of $\tilde{Q}_{k-1}$ in~\eqref{eq:virtual_q}, if $\forall a'\in\cA$, $\phi(s, a')\in\cH$ , then $\pi_{k}(a|s) = \tilde\pi_{k}(a|s)$. This means that if suffices to show that $\forall s\in T_{\pi_{k}}^n(z_s, z_a)$, $\forall a'\in\cA$, $\phi(s, a')\in\cH$, which is a direct consequence of the fact that this is the last loop in the algorithm and the $\mathsf{RolloutWithUncertainty}$ subroutine does not return $\mathsf{uncertain}$ status.
\end{proof}

With this lemma, Lemma~\ref{lem:est_error} and the definition of $\tilde{Q}_{k-1}$, we know that for any $(s, a)\in\cS\times\cA$,
\begin{align}\label{eq:tilde_infty}
| \tilde{Q}_{k-1}(s, a) - Q_{\tilde{\pi}_{k-1}} (s, a)| \le b\sqrt{\lambda \tau} + \big(\epsilon + \frac{\gamma^{n+1}}{1-\gamma}\big) \sqrt{\frac{d(1+\tau)}{\lambda \tau}}:=\eta.
\end{align}
This is because when $\phi(s, a)\in\cH$, this inequality holds due to Lemma~\ref{lem:est_error} and otherwise $\tilde{Q}_{k-1}(s, a) = Q_{\tilde{\pi}_{k-1}} (s, a)$. Then, the virtual algorithm can be considered as API with an approximate Q-function that is close to the true Q-function in $\ell_\infty$ norm. We use the following results for API, which is a direct consequence of the results in~\citet{munos2003error,farahmand2010error}, and is also stated in~\citet{lattimore2020learning}. 
\begin{lemma}\label{lem:api}
Suppose that we run $K$ approximate policy iterations and generate a sequence of policies $\pi_0, \pi_1, \ldots, \pi_K$. 
Suppose that for every $k=1,2,\ldots, K$, in the $k$-th iteration, we obtain a function $\tilde{Q}_{k-1}$ such that, $\|\tilde{Q}_{k-1} - Q_{\pi_{k-1}}\|_\infty\le \eta$, and choose $\pi_k$ to be greedy with respect to $\tilde{Q}_{k-1}$. Then
\[
\|Q^* - Q_{\pi_{K}}\|_\infty \le \frac{2\eta}{1-\gamma} + \frac{\gamma^K}{1-\gamma}.
\]
\end{lemma}
%In the following, we let $\eta:=b\sqrt{\lambda \tau} + \big(\epsilon + \frac{\gamma^{n+1}}{1-\gamma}\big) \sqrt{\frac{d(1+\tau)}{\lambda \tau}}$ be the $\ell_\infty$ distance between $\tilde{Q}_{k-1}$ and $Q_{\tilde{\pi}_{k-1}}$.
According to Lemma~\ref{lem:api},
\begin{equation}\label{eq:tilde_q_result}
\|Q^* - Q_{\tilde\pi_{K-2}}\|_\infty \le  \frac{2\eta}{1-\gamma} + \frac{\gamma^{K-2}}{1-\gamma}.
\end{equation}
The following lemma translates the gap in Q-functions to the gap in value.
\begin{lemma}\label{lem:api_value}
\citep{singh1994upper} Let $\pi$ be greedy with respect to a function $Q$. Then for any state $s$,
\[
V^*(s) - V_\pi(s) \le \frac{2}{1-\gamma}\|Q^*-Q\|_\infty.
\]
\end{lemma}
Therefore, for the virtual API algorithm,
\[
V^*(\rho) - V_{\tilde{\pi}_{K-1}}(\rho) \le \frac{4\eta}{(1-\gamma)^2} + \frac{2\gamma^{K-2}}{(1-\gamma)^2}.
\]

Recall that in the first step of the algorithm, we add a state-action pair $(\rho, a)$, with an arbitrary $a\in\cA$ to the core set. Thus, when the algorithm terminates, we know that for all $a\in\cA$, $\phi(\rho, a)\in\cH$, and thus $\pi_{K-1}(\rho) = \tilde\pi_{K-1}(\rho)$. According to the proof of Lemma~\ref{lem:virtual_api}, we also know that $w_{K-1} = \tilde{w}_{K-1}$. Therefore, $Q_{K-1}(\rho, \pi_{K-1}(\rho)) = \tilde{Q}_{K-1}(\rho, \tilde\pi_{K-1}(\rho))$. This implies that
\begin{align}
|V_{\pi_{K-1}}(\rho) - V_{\tilde\pi_{K-1}}(\rho)| =&  |Q_{\pi_{K-1}}(\rho, \pi_{K-1}(\rho)) - Q_{\tilde\pi_{K-1}}(\rho, \tilde\pi_{K-1}(\rho))| \nonumber \\
\le & |Q_{\pi_{K-1}}(\rho, \pi_{K-1}(\rho)) - Q_{K-1}(\rho, \pi_{K-1}(\rho))| \nonumber \\
&+ |Q_{\tilde\pi_{K-1}}(\rho, \tilde\pi_{K-1}(\rho)) - \tilde{Q}_{K-1}(\rho, \tilde\pi_{K-1}(\rho))| \nonumber \\
\le & 2\eta, \label{eq:q_to_v}
\end{align}
where the last inequality is due to Lemma~\ref{lem:est_error}. This yields
\begin{align}\label{eq:final_v}
    V^*(\rho) - V_{{\pi}_{K-1}}(\rho) \le \frac{6\eta}{(1-\gamma)^2} + \frac{2\gamma^{K-2}}{(1-\gamma)^2}.
\end{align}
Our final step is to choose the appropriate parameters $\lambda$, $\tau$, $K$, and $n$. We consider two cases.
The first case is when Assumption~\ref{asm:linear_realizability} holds, i.e., $\epsilon=0$. In this case, we hope to ensure that $V^*(\rho) - V_{{\pi}_{K-1}}(\rho) \le \kappa$ for an arbitrarily small $\kappa >0$. According to the definition of $\eta$ in Eq.~\eqref{eq:tilde_infty}, it suffices to guarantee that
\begin{align}\label{eq:final_gap_exact}
\frac{6b\sqrt{\lambda \tau}}{(1-\gamma)^2}
+  \frac{6\gamma^{n+1}}{(1-\gamma)^3} \sqrt{\frac{d(1+\tau)}{\lambda \tau}}
+ \frac{2\gamma^{K-2}}{(1-\gamma)^2} \le \kappa.
\end{align}
It can be verified that by choosing $\tau = 1$, $\lambda = \frac{\kappa^2(1-\gamma)^4}{324 b^2}$, $K = 2+\frac{2\log(\frac{3}{\kappa(1-\gamma)})}{1-\gamma}$, and $n=\frac{5\log(\frac{4db}{\kappa(1-\gamma)})}{1-\gamma}$, Eq.~\eqref{eq:final_gap_exact} can be guaranteed.
The second case is when Assumption~\ref{asm:linear_realizability_prox} holds, i.e., $\epsilon > 0$. In this case, the final gap $V^*(\rho) - V_{\pi_{K-1}}(\mu)$ is
\begin{align}\label{eq:final_gap_prox}
    V^*(\rho) - V_{\pi_{K-1}}(\mu) \le \frac{6b\sqrt{\lambda \tau}}{(1-\gamma)^2}
+  \frac{6}{(1-\gamma)^2} \big(\epsilon + \frac{\gamma^{n+1}}{1-\gamma}\big) \sqrt{\frac{d(1+\tau)}{\lambda \tau}}
+ \frac{2\gamma^{K-2}}{(1-\gamma)^2}.
\end{align}
Now we try to minimize the right hand side of~\eqref{eq:final_gap_prox}. It can be verified that if we choose $\tau = 1$, $\lambda = \frac{\epsilon}{b}\sqrt{2d}$, $K=2 + \frac{1}{1-\gamma} \log\big(\frac{1}{\epsilon^{1/2}b^{1/2}d^{1/4}}\big)$, and $n=\frac{1}{1-\gamma}\log(\frac{1}{\epsilon(1-\gamma)})$, then the right hand side of~\eqref{eq:final_gap_prox} is upper bounded by $\frac{24\epsilon^{1/2}b^{1/2}d^{1/4}}{(1-\gamma)^2}$


% some removed comments, just in case.
%For instance, it captures the ``saved files'' feature in video games that allows players to record player progress and resume from the saved points later on.

% (1) the agent is allowed to obtain samples from the initial state distribution and query the simulator with the initial state paired with an arbitrary action; and (2)
% I think we don't have to mention that the agent is allowed to sample from the initial state distribution here, since in most parts of the paper we will assume that the initial state is deterministic. We will discuss random initial state in the appendix..


%{\botao (Botao: this might be a bit misleading? Since our guarantee is also for local optimality.)}\dong{That's a good point. Is the current version better?}


%\dong{Should we say linear realizability of all deterministic policies? We don't plan to add Politex in the first arXiv version anyway.}{\botao Botao: to be more rigorous, should be the realizability for all stationary deterministic policies? }\dong{By stationary, did you mean the policy is independent of the time step? I think this is kind of implied by the definition but we can mention that in the preliminary section.} {\botao Botao: yes. I chat with Tor on this. He didn't believe realizability of deterministic and stationary policies can imply the realizability of stochastic policies.}

% Assuming $Q_\pi$ realizability and access to the full feature matrix, \cite{lattimore2020learning, du2020good} derived an $O(d/\varepsilon^2(1-\gamma)^4)$ query complexity bound.  


% Assuming $Q_\pi$ realizability and access to the full feature matrix, \cite{lattimore2020learning, du2020good} derived an $O(d/\varepsilon^2(1-\gamma)^4)$ query complexity bound.  


% {\botao (Botao: we use $\kappa$ as the final sub-optimality gap. Is the same as $\varepsilon$, right?)}{\botao (Botao: special case? Ours is more general?)} \dong{I think our case is more restrictive in the sense that we cannot query an arbitrary state-action pair. I swapped the order of the related work back to generative model, local access, online. They are reversely ordered by the ``access freedom'' now.}

%where $\varepsilon$ is the average regret and $\Delta_{\text{gap}}$ is the sub-optimality gap.

% {\botao (Botao: shall we unify $H=1/(1-\gamma)$? But for regret, it might not be appropriate to write $1/(1-\gamma)$...)} \dong{Yeah I think we are being vague between episodic and discounted. We can clarify in the beginning of this section.}


% Currently this remark is moved to the related work section.
% \paragraph{Remark}
% As shown in \cite{zanette2020learning}, $Q_{\pi}$-realizability is strictly weaker than linear MDP assumption but obivously is stronger than $Q^*$-realizability.

%{\botao (According to Csaba's suggestion, we may wonder if the realizability of all the stochastic policy can be relaxed to only deterministic policy if we want to use politex. There is no benefit to switch to politex in the fully realizable case?) }\dong{Yes, for exactly realizable case politex does not seem to bring additional benefit.}

%\dong{We should extend this to $ | Q_\pi(s, a) - w_\pi^\top \phi(s, a)| \le \epsilon $.} {\botao Botao: do we need to know $\epsilon$?} \dong{Yeah maybe, I think we will need to know $\epsilon$ to choose $\lambda$ and $\tau$ optimally...}

% A basic question in the formulation above is how the agent accesses the reward function, the probability transition kernel, and the feature vectors. 
%Here, we consider the setting known as \emph{reinforcement learning with a generative model}. In this setup, t
% We assume that the agent can query a generative model, also called a simulator, with a state-action pair $(s, a)$, and the generative model returns the feature vector $\phi(s, a)$, the reward value $r(s, a)$, and a sample of next state $s' \sim P(s, a)$. We aim to understand the number of times that the agent needs to query the generative model in order to learn a good policy $\pi$ such that $V^* - V_\pi(\rho)$ is small.

%Note that a major difference between our generative model setup and several prior works~\citep{} is that we take the cost of querying the feature vectors into account. On the contrary, prior works typically assume that the feature vectors are provided to the agent before the algorithm starts, and the agent can use the entire feature matrix to learn an optimal design or a barycentric spanner. As mentioned, the computational complexity of such procedure is usually polynomial in the state space and thus the methods are inefficient with large state space.

%We now proceed to describe our algorithm. Since the Q-functions are linear in the features, we also parameterize the policies using linear functions. More specifically, 

% {\botao (Botao: in the main theorem, we didn't write explicitly for the order dependency on $1/(1-\gamma)$.)}\dong{No, I think in the main theorem we mostly want to say that the complexities are polynomial. We clarify these $(\frac{1}{1-\gamma})^{20}$ things in the discussion.}

% \todoc{
% So what is missing here or somewhere else (intro?) is the following:
% For simulators, we can distinguish between them based on access.
% Random access means that the planner is given a list of state action pairs and can name any of them to get a random transition.
% Local access means access to states previously encountered (reset to previously ``seen'' states, implementable with checkpointing).
% Online access means that the simulation state can only be reset to the initial state (or distribution) or moved to a next random state given an action. 
% Random access is often unavailable. E.g. in robotics, a superset of the state space may be known but  some configurations may be forbidden because of collisions.
% As far as planning problems are considered, we can distinguish between 
% online planning (formerly local planning), where the planner implements a `getaction' function and the induced policy must be a good one,
% and
% offline planning where the planner implements a `getpolicy' function.
% Subdividing this into two, there is global offline planning where the `getpolicy' function must return a policy that is good for every initial state and local planning, when getpolicy is provided an initial state distribution and the policy returned must be a good one only for that distribution. We should probably explain this in the intro.
% }

We restate the core set construction process in the following way with slightly different notation. We begin with $\Phi_0 = 0$. In the $t$-th step, we have a core set with feature matrix $\Phi_{t-1}\in\R^{(t-1)\times d}$. Suppose that we can find $\phi\in\R^d$, $\|\phi\|_2 \le 1$, such that
\begin{align}\label{eq:new_feature}
\phi^\top (\Phi_{t-1}^\top \Phi_{t-1} + \lambda I)^{-1} \phi > \tau,
\end{align}
then we let $\Phi_t := [\Phi_{t-1}^\top~~ \phi]^\top\in\R^{t \times d}$, i.e., we add a row at the bottom of $\Phi_{t-1}$. Otherwise we terminate this process. We define $\Sigma_t := \Phi_t^\top\Phi_t + \lambda I$.

To show that the process above must terminate within $\frac{d(1+\tau)}{\lambda \tau^2}$ steps, we focus on the trace of $\Sigma_t^{-1}$. Since $\forall t, \Sigma_t^{-1} \succeq 0$, $\tr(\Sigma_t^{-1}) \ge 0$. We also know that $\tr(\Sigma_0^{-1}) = \frac{d}{\lambda}$. We show that after each step, $\tr(\Sigma_t^{-1})$ decreases by at least $\frac{\tau^2}{1+\tau}$, i.e., for any $t$,
\begin{align}\label{eq:decrease}
\tr(\Sigma_{t}^{-1}) \le \tr(\Sigma_{t-1}^{-1}) - \frac{\tau^2}{1+\tau},
\end{align}
then after at most $\frac{d(1+\tau)}{\lambda\tau^2}$ steps, the algorithm must stop. In the following we focus on proving~\eqref{eq:decrease}.

Write the eigendecomposition of $\Sigma_{t-1}$ as $\Sigma_{t-1}=V\Lambda V^\top$, where $V$ is an orthonormal matrix, and $\Lambda := \diag(\lambda_1, \ldots, \lambda_d)$. Then
\begin{align}\label{eq:trace_tm1}
    \tr(\Sigma_{t-1}^{-1}) = \tr(\Lambda^{-1}) = \sum_{i=1}^d \lambda_i^{-1}.
\end{align}
Let $\phi$ be a vector such that~\eqref{eq:new_feature} holds, and let $\alpha$ be a vector such that $\phi = V \alpha$. Since $\|\phi\|_2 \le 1$, we know $\|\alpha\|_2\le 1$. Moreover, by~\eqref{eq:new_feature}, we know that
\[
\alpha^\top V^\top V\Lambda^{-1} V^\top V \alpha > \tau, 
\]
which implies that
\begin{align}\label{eq:alpha_condi}
    \sum_{i=1}^d \alpha_i^2\lambda_i^{-1} > \tau.
\end{align}
Now we write $\Sigma_t^{-1}$ as:
\begin{align}
    \Sigma_t^{-1} & = (\Phi_{t-1}^\top \Phi_{t-1} + \phi\phi^\top + \lambda I)^{-1}\nonumber \\
    &= V (\Lambda + \alpha\alpha^\top)^{-1} V^\top \nonumber \\
    &= V(\Lambda^{-1} - \Lambda^{-1} \alpha(1+\alpha^\top\Lambda^{-1}\alpha)^{-1}\alpha^\top \Lambda^{-1})V^\top,
    \label{eq:woodbury}
\end{align}
where the last equation is due to Woodbury matrix identity~\citep{woodbury1950inverting}. This yields
\begin{align}
    \tr(\Sigma_t^{-1}) &= \tr(\Lambda^{-1}) - \tr(\Lambda^{-1} \alpha(1+\alpha^\top\Lambda^{-1}\alpha)^{-1}\alpha^\top \Lambda^{-1}) \nonumber \\
    &=\tr(\Sigma_{t-1}^{-1}) - (1+\alpha^\top\Lambda^{-1}\alpha)^{-1}\tr(\Lambda^{-1}\alpha \alpha^\top \Lambda^{-1}) \nonumber \\
    &=\tr(\Sigma_{t-1}^{-1}) - (1+\alpha^\top\Lambda^{-1}\alpha)^{-1}\alpha^\top\Lambda^{-2}\alpha \nonumber \\
    &=\tr(\Sigma_{t-1}^{-1}) - \frac{\sum_{i=1}^d \alpha_i^2\lambda_i^{-2}}{1+\sum_{i=1}^d \alpha_i^2\lambda_i^{-1}}. \label{eq:decrease_trace}
\end{align}
According to Cauchy–Schwarz inequality, we know that
\[
\left(\sum_{i=1}^d \alpha_i^2\right) \left(\sum_{i=1}^d \alpha_i^2\lambda_i^{-2}\right) \ge \left(\sum_{i=1}^d \alpha_i^2 \lambda_i^{-1}\right)^2,
\]
which yields
\begin{align}\label{eq:cauthy}
    \sum_{i=1}^d \alpha_i^2\lambda_i^{-2} \ge \frac{\left(\sum_{i=1}^d \alpha_i^2 \lambda_i^{-1}\right)^2}{\sum_{i=1}^d \alpha_i^2} \ge \left(\sum_{i=1}^d \alpha_i^2 \lambda_i^{-1}\right)^2,
\end{align}
where in the second inequality we use the fact that $\|\alpha\|_2\le 1$. We combine~\eqref{eq:decrease_trace} and~\eqref{eq:cauthy} and obtain
\[
\tr(\Sigma_t^{-1}) \le \tr(\Sigma_{t-1}^{-1}) - \frac{\left(\sum_{i=1}^d \alpha_i^2 \lambda_i^{-1}\right)^2}{1+\sum_{i=1}^d \alpha_i^2\lambda_i^{-1}}.
\]
Notice that the function $\frac{x^2}{1+x}$ monotonically increases when $x\in(0, +\infty)$. Then using~\eqref{eq:alpha_condi}, we know that
\[
\tr(\Sigma_t^{-1}) \le \tr(\Sigma_{t-1}^{-1}) - \frac{\tau^2}{1+\tau},
\]
which validates~\eqref{eq:decrease} and thus completes the proof.
